On the Relationship of Optimal State Feedback and Disturbance Response Controllers

This paper studies the relationship between state feedback policies and disturbance response policies for the standard Linear Quadratic Regulator (LQR). For open-loop stable plants, we establish a simple relationship between the optimal state feedback controller $u_t=K_\star x_t$ and the optimal disturbance response controller $u_t=L^{(H)}_{\star;1}w_{t-1}+\cdots+L^{(H)}_{\star;H}w_{t-H}$ with $H$-order. Here $x_t, w_t, u_t$ stands for the state, disturbance, control action of the system, respectively. Our result shows that $L_{\star,1}^{(H)}$ is a good approximation of $K_\star$ and the approximation error $\|K_\star - L_{\star,1}^{(H)}\|$ decays exponentially with $H$. We further extend this result to LQR for open-loop unstable systems, when a pre-stabilizing controller $K_0$ is available.

==> Equivalence_2_parameterizations/Sections/Preliminaries.tex <==
\section{PROBLEM SETTINGS AND PRELIMINARIES}\label{sec:preliminaries}
We consider the standard infinite-horizon discrete time linear quadratic regulator (LQR) problem
\begin{equation}\label{eq:LQR}
\begin{split}
\min_{\{u_t\}_{t=0}^{\infty}}&\lim_{T\to\infty} \frac{1}{T}\mathbb{E}\sum_{t=0}^{T-1}x_t^\top Q x_t + u_t^\top Ru_t + 2 u_t^\top S x_t\\
 s.t.~~ x_{t+1} &= Ax_t + Bu_t + w_t, ~~w_t\sim\mathcal{N}(0,I),
\end{split}
\end{equation}
where $x_t\in \bR^{n_x}, u_t\in \bR^{n_u}$ denote the state vector and control input respectively. Here we consider the case that \eqref{eq:LQR} represents the joint dynamics of $N$ agents $[N]= \{1,2,\dots,N\}$, i.e., $x_t$ and $u_t$ can be written as
\begin{align*}
    x_{t} &= [x_{t}^{1\top}, x_{t}^{2\top}, \cdots, x_t^{N\top}]^\top,\\
    u_t &= [u_t^{1\top}, u_t^{2\top}, \cdots, u_t^{N\top}]^\top,
\end{align*}
where $x_t^i\in \bR^{n_x^i}, u_t^i\in \bR^{n_u^i}$ represents the state and control input of agent $i$. The dimension of the joint state and control input vectors satisfies $n_x = \sum_{i=1}^N n_x^i, n_u = \sum_{i=1}^N n_u^i$. The dynamic of individual agents' state $x_t^i$'s can be written as
\begin{equation}\label{eq:dynamic-x-i}
    x_{t+1}^i= \sum_{j\in [N]}[A]_{ij}x_{t}^j + [B]_{ij}u_t^j,
\end{equation}
and the stage cost $x_t^\top Qx_t + u_t^\top Ru_t + 2 u_t^\top S x_t$ can be written as
\begin{equation*}
    %x_t^\top Qx_t + u_t^\top Ru_t + 2 u_t^\top S x_t = 
    \sum_{i,j=1}^N x_t^{i\top} [Q]_{ij}x_t^j + u_t^{i\top} [R]_{ij}u_t^j + 2u_t^{i\top} [S]_{ij}x_t^j.
\end{equation*}
Here the submatrix notation $[X]_{ij}$ denotes the submatrix of $X$ where its row indexes corresponds to the role indexes of agent $i$ and its column indexes corresponds to the indexes of agent $j$.\footnote{By indexes of agent $i$, we mean that, if the total index length is $n_x$, then the indexes of agent $i$ is of range $\big[\sum_{j=1}^{i-1} n_x^i+1, \sum_{j=1}^{i} n_x^i\big]$. And the same definition also applies for total index length of $n_u$.}

Throughout the paper, we use $\|\cdot\|$ to denote the $\ell_2$ norm of a vector as well as the induced $\ell_2$ norm of a matrix. $\lmax(X), \lmin(X)$ denotes the maximum and minimum eigenvalue of a square matrix $X$ respectively.

\noindent\textbf{Spatially exponential decaying structure.} In this paper we assume that there's a distance function defined on the set of $N$-agents, i.e. $\dist(\cdot,\cdot): [N]\times[N]\rightarrow \mathbb{R}^{\ge 0}$, such that $\dist(i,j) = \dist(j,i)$, and that triangle inequality holds $\dist(i,j)\le \dist(i,k) + \dist(k,j),~\forall i,j,k\in [N]$. For example, if the $N$ agents are embedded on an un-directed graph, then $\dist(i,j)$ can be taken as the graph distance, which is the length of the shortest path from agent $i$ to $j$. 
\begin{definition}[Spatially exponential decaying (SED)]\label{def:SED}
A matrix $X\in\bR^{n'\times n''}$ ($n',n'' = n_x$ or $n_u$) is $(c, \gamma)$-spatially exponential decaying (SED) if
\begin{equation*}
    \|[X]_{ij}\|\le c\cdot e^{-\gamma \dist(i,j)}, ~~\forall~ i,j\in [N].
\end{equation*}
\end{definition}
%\lina{another way to define the exponential decaying is $c\cdot \rho^{\text{dist}(i,j)}$ here $\rho$ is $e^{-\gamma}$. I think $c\rho^k$ is more straightforward and it is more aligned with discrete time system.} \textcolor{blue}{Maybe change it to $(c, e^{-\gamma})$-SED?}

We make the following spatially decaying assumption on the system parameters $A,B,Q,R,S$:
\begin{assump}[SED system]\label{assump:exponential-decay}
There exists $\gammasys  >0$ and constant $a,b,q,r,s>0$ such that $A,B,Q,R,S$ are $(a,\gammasys ), (b,\gammasys ), (q,\gammasys ), (r,\gammasys ), (s,\gammasys )$-SED respectively. Here for convenience, we assume without loss of generality that
$a,b,q,r\ge 1$.
\end{assump}
% {\color{blue} TODO: why we care about SED system, maybe even change the examples to continuous time, and then do discretization to make the story more reasonable}

Assumption \ref{assump:exponential-decay} implies that both the system dynamics as well as the quadratic cost are decoupled across agents to a certain extend. From \eqref{eq:dynamic-x-i}, if $\dist(i,j)$ is large, then Assumption \ref{assump:exponential-decay} guarantees that $x_j, u_j$ have exponentially small effect on the dynamics of $x_i$.

\noindent \textbf{Why SED?}
%\lina{lina needs to revise the following discussion on why sed. may start with a more general discription (e.g., spatial invariant system, pde, etc), saying that they motivated us to study this. Then bring the more specific example on sparse continuous dynamical systems and talk about discretization.} 
One important motivation of studying SED systems arises from the continuous time network LQR problem considered in vast literature (e.g. \cite{Bamieh02}):
\begin{align*}
\min_{\{u(t)\}} &\int_0^{+\infty} x(t)^\top Q_cx(t) + u(t)^\top R_cu(t)\\
&\dot{x} = A_c x + B_c u,
\end{align*}
In many applications, such as thermal dynamics (see Example \ref{example:circle} below), $A_c, B_c$ are sparse matrices with $[A_c]_{ij}, [B_c]_{ij} = 0$ if $\dist(i,j) >1$, i.e., the corresponding matrices entries will be zero if $i,j$ are not neighbors of each other. 

In order to practically solve the continuous time control problem, discretization is needed. Standard result shows that
\begin{align*}
    x(t+\Delta t) = e^{\Delta t A_c}x(t) + \left(\int_0^{\Delta t}e^{(t+\Delta t - s)A_c}B_cu(s)ds\right),
\end{align*}
thus we could apply the following discretization scheme .
\begin{align}\label{eq:discretization}
    A \!=\! e^{\Delta t A_c}, ~~B\!=\! \left(\!\int_0^{\Delta t}\!\!\!e^{sA_c}ds\!\right) B_c, ~~Q \!=\! \Delta t Q_c,~~ R \!=\! \Delta t R_c
\end{align}
Note that this discretization scheme is more accurate compared with doing forward Euler scheme cite??. However, for discretization scheme \eqref{eq:discretization} the sparsity structure is not preserved for $A,B$. Fortunately, it can be shown that although $A,B$ are not sparse, they are SED with respect to the original graph distance (see Proposition \ref{prop:discretize-SED} in Appendix \ref{apdx:why-SED}). Thus, in order to handle this type of problems, we consider a broader setting of SED systems rather than sparse network systems in this paper.


%  While this work considers discrete time LQR problem, most practical systems are continuous time in nature. Thus in order for our results to apply to more practical cases, discretization of continuous time dynamics is necessary. For a continuous time linear system
% \begin{align*}
% \min_{\{u(t)\}} &\int_0^{+\infty} x(t)^\top Q_cx(t) + u(t)^\top R_cu(t)\\
% &\dot{x} = A_c x + B_c u,
% \end{align*}
% standard result shows that
% \begin{align*}
%     x(t+\Delta t) = e^{\Delta t A_c}x(t) + \left(\int_0^{\Delta t}e^{(t+\Delta t - s)A_c}B_cu(s)ds\right) 
% \end{align*}
% thus we could apply the following discretization scheme for the examples considered in this section.
% \begin{align}\label{eq:discretization}
%     A \!=\! e^{\Delta t A_c}, ~~B\!=\! \left(\!\int_0^{\Delta t}\!\!\!e^{sA_c}ds\!\right) B_c, ~~Q \!=\! \Delta t Q_c,~~ R \!=\! \Delta t R_c
% \end{align}
% In many applications, such as thermal dynamics (see Example \ref{example:circle} below), $A_c, B_c$ are sparse matrices with $[A_c]_{ij}, [B_c]_{ij} = 0$ if $\dist(i,j) >1$, i.e., $i,j$ are not neighbors of each other. However, for discretization scheme \eqref{eq:discretization} the sparsity structure is not preserved for $A,B$. For these types of systems, it can be shown that although $A,B$ are not sparse, they are SED with respect to the original graph distance .


\begin{example}[Heat equation on a circle $\mathbb{Z}_N$]\label{example:circle}
Consider the case where the $N$ agents are located on a circle $\mathbb{Z}_N$, where agent $i$ is only connected with $i-1$ and $i+1$ (modular $N$). The heat equation dynamic is defined as:
\begin{equation*}
    \dot x^i = -2x^i + x^{i+1} + x^{i-1} + b_i u^i,
\end{equation*}
thus $A_c = -L$, where where $L$ is the graph Laplacian of $\mathbb{Z}_N$, and $B_c = \diag(\{b_i\}_{i=1}^N)$ is a diagonal matrix whose diagonal entries are $b_i$'s.
The control objective is to let the state vector goes to zero while keeping the control energy low, which can be modeled as
\begin{equation*}
    \int_0^{+\infty} \sum_{i=1}^N q_i {x(t)^i}^2 + r_i {u(t)^i}^2
\end{equation*}
thus $Q_c, R_c$ matrices in this setting are $Q_c = \diag(\{q_i\}_{i=1}^N), R_c = \diag(\{r_i\}_{i=1}^N)$. Since $A_c, B_c, Q_c, R_c$ are all sparse matrices, i.e. $\|[A_c]_{ij}\| = 0$ is $i,j$ are not neighbors on the circle $\mathbb{Z}_N$, we can apply discretization scheme \eqref{eq:discretization} to get the corresponding discrete time LQR with system matrix $A,B,Q,R$. Proposition \ref{prop:discretize-SED} implies that $A,B,Q,R$ are SED.
% \begin{equation*}
%      x_{t+1}^i = x_t^i + \eta\left(-2x_t^i + x_t^{i+1} + x_t^{i-1}  + b_i u_t^i\right),
% \end{equation*}
% thus $A = I-\eta L$, where $L$ is the graph Laplacian of $\mathbb{Z}_N$, and $B = \eta \diag(\{b_i\}_{i=1}^N)$ is a diagonal matrix whose diagonal entries are $\eta b_i$'s.
% The control objective is to let the state vector goes to zero while keeping the control energy low, which can be modeled as
% \begin{equation*}
%     \min \lim_{T\to\infty}\frac{1}{T} \sum_{t=1}^T\sum_{i=1}^N q_i {x_t^i}^2 + r_i {u_t^i}^2,
% \end{equation*}
% thus $Q, R$ matrices in this setting are $Q = \diag(\{q_i\}_{i=1}^N), R = \diag(\{r_i\}_{i=1}^N)$.
% In this example with small $\eta<1$, we can set $\gammasys  = \log(\frac{1}{\eta})$, $a=1$, $b=\max\{\eta\max_i b_i,1\}$, $q=\max\{\max_i q_i,1\}$ and $r=\max\{\max_i r_i,1\}$ in Assumption \ref{assump:exponential-decay}.
\end{example}

% \begin{example}[Heat equation on a graph $\mathcal{G}$]\label{example:random-graph}
% We can also generalize the heat equation in Example \ref{example:circle} to any undirected graph $\mathcal{G} = \{V, E\}$, where $V = [N]$ is the vertex set of the graph, $E = \{w_{ij}\}$ is the edge set and $w_{ij}\ge0$ is the weight of the edge connecting agent $i$ and $j$ ($w_{ij} = 0$ if there is no edge connecting the two agents). The heat equation dynamic is then defined as
% \begin{align*}
%      x_{t+1}^i = x_t^i + \eta\left(-w_{i}x_t^i + \sum_{j\neq i} w_{ij}x_t^j  + b_i u_t^i\right),\\\quad \text{where }w_{i} := \sum_{j\neq i} w_{ij}.\qquad\qquad\qquad
% \end{align*}
% The new dynamic together with the control objective in Example \ref{example:circle} has the same expressions for $A,B,Q,R$ and their SED parameters, while $L$ denotes the weighted graph Laplacian, and $\gammasys $ is changed to $\gammasys  = \min_{i\ne j}\frac{-\ln(\eta w_{ij})}{\dist(i,j)}$.
% \end{example}

% \noindent\textbf{Optimal control gain $K$ and optimal cost-to-go matrix $P$} The solution to problem \eqref{eq:LQR} is known to be solved by a linear state feedback controller $u_t = -Kx_t$, where 
% \begin{equation}\label{eq:F-expr}
%     K = (R+B^\top P B)^{-1}(B^\top P A+S).
% \end{equation}
% Here, the cost-to-go matrix $P$ is known to satisfy the algebraic Ricatti equation
% \begin{equation}\label{eq:ricatti-eq}
%     P \!=\! A^\top P A - (A^\top PB+S^\top)(R + B^\top PB)^{-1}(B^\top PA+S) + Q.
% \end{equation}
% As mentioned in the introduction, one major motivation of our work is to answer the important question of whether an SED system that satisfies Assumption \ref{assump:exponential-decay} still obtains the optimal LQR controller $K$ which is also SED. However, answering the question is not trivial. One of the major technical difficulties is that the algebraic Ricatti equation \eqref{eq:ricatti-eq} is a \textit{nonlinear} matrix equation, and it is hard to verify how the spatially decaying structure is preserved given that the matrix coefficients $A,B,Q,R,S$ in \eqref{eq:ricatti-eq} are SED. This observation inspires us to think about the problem from a different perspective --- doing convex reparameterization of \eqref{eq:LQR} using disturbance response. The reason that we start with disturbance response is that it translates the nonlinear equation \eqref{eq:ricatti-eq} to a linear equation (see \eqref{eq:L-tilde-eq} in Section \ref{sec:disturbance-response}), whose structure is much easier to analyze compared with the nonlinear Ricatti equation. Thus, instead of directly analyzing the SED structure of $K$, we first study the SED structure for disturbance feedback and then translate the result back to state feedback. 

% \textbf{Organization of the paper:} Given the above intuition, this paper is organized as follows. Section \ref{sec:disturbance-response} introduces the disturbance response parameterization and calculates the optimal finite-truncated response, which turns out to be the solution of a linear matrix equation \eqref{eq:L-tilde-eq}; following this observation, Section \ref{sec:MK-HK-LK-structure} analyzes the SED structure of this linear matrix equation and shows that the optimal finite-truncated response is SED. Section \ref{sec:translate-back-to-state-feedback} translates the result from disturbance feedback to state feedback and shows that the optimal state feedback control gain $K$ is also SED.

% % \textcolor{blue}{TODO: maybe add some preliminary on disturbance response, can just state the formulation. Three main message (Hmmm actually on second thought I am not sure whether we should include this into the preliminary. Probably I would prefer the current structure)}

% In order to leverage disturbance feedback parameterization, we further assume that $A$ is exponentially stable (Assumption \ref{assump:A-exponential-stable}). We would also like to note that this assumption could be further extend to the unstable case with stabilizability assumption %We would also like to note that this Assumption seems necessary. For $A$ that is unstable, we give a counter-example in Appendix \ref{apdx:counter-example} showing that the optimal $K$ is not spatially decaying even though the system satisfies Assumption \ref{assump:exponential-decay}, suggesting that more assumptions are needed for unstable $A$'s to obtain a SED optimal controller. Due to time constraints, we mark it as one of the future works.
% \begin{definition}[$(\tau,e^{-\rho})$-stability] For $\tau\ge1, \rho>0$, we define a matrix $A$ as $(\tau, e^{-\rho})$-stable if
% \begin{equation*}
%     \|A^k\|\le \tau e^{-\rho k}.
% \end{equation*}
% \end{definition}

% \begin{assump}[Open-loop and Closed-loop Stability]\label{assump:A-exponential-stable}
% There exists $\tau\ge 1,\rho>0$ both $A$ and $A-BK$ are $(\tau, e^{-\rho})$-stable, where $K$ is the optimal state feedback control gain of \eqref{eq:LQR}.
% \end{assump}

